A multi-wavelength investigation of PSR J2229+6114 and its pulsar wind nebula in the radio, X-ray, and gamma-ray bands

G106.3$+$2.7, commonly considered a composite supernova remnant (SNR), is characterized by a boomerang-shaped pulsar wind nebula (PWN) and two distinct ("head" & "tail") regions in the radio band. A discovery of very-high-energy (VHE) gamma-ray emission ($E_\gamma > 100$ GeV) followed by the recent detection of ultra-high-energy (UHE) gamma-ray emission ($E_\gamma > 100$ TeV) from the tail region suggests that G106.3$+$2.7 is a PeVatron candidate. We present a comprehensive multi-wavelength study of the Boomerang PWN (100" around PSR J2229+6114) using archival radio and Chandra data obtained from two decades ago, a new NuSTAR X-ray observation from 2020, and upper limits on gamma-ray fluxes obtained by Fermi and VERITAS observatories. The NuSTAR observation allowed us to detect a 51.67 ms spin period from the pulsar PSR J2229+6114 and the PWN emission characterized by a power-law model with $\Gamma = 1.52\pm0.06$ up to 20 keV. Contrary to the previous radio study by Kothes et al. 2006, we prefer a much lower PWN B-field ($B\sim3$ $\mu$G) and larger distance ($d \sim 8$ kpc) based on (1) the non-varying X-ray flux over the last two decades, (2) the energy-dependent X-ray PWN size resulting from synchrotron burn-off and (3) the multi-wavelength spectral energy distribution (SED) data. Our SED model suggests that the PWN is currently re-expanding after being compressed by the SNR reverse shock $\sim 1000$ years ago. In this case, the head region should be formed by GeV--TeV electrons injected earlier by the pulsar propagating into the low density environment.

==> old_bibliography.tex <==
\begin{thebibliography}{}

% 4FGL
\bibitem[Abdollahi et al.(2020)]{Abdollahi-2020} Abdollahi, S. \& others\ 2020, \apj, 247, 33

% Abeysekara HAWC paper
\bibitem[Abeysekara et al.(2020)]{Abeysekara-2020} Abeysekara, A. U. \& Albert, A. \& Alfaro, R. \& Angeles Camacho, J. R. \& Arteaga-Velázquez, J. C. \& Arunbabu, K. P. \& Avila Rojas, D. \& Ayala Solares, H. A. \& Baghmanyan, V. \& Belmont-Moreno, E. \& et al.\ 2020, \apj, 124, 2.

% Fermi Large Area Telescope Third Source Catalog - NASA/ADS
\bibitem[Acero et al.(2015)]{Acero-2015} Acero, F., Ackermann, M., Ajello, M., et al.\ 2015, \apjs, 218, 23. doi:10.1088/0067-0049/218/2/23

% HESS Crab
\bibitem[Aharonian et al.(2006)]{Aharonian-2006} Aharonian, F. et al.\ 2006, A&A, 457, 899-915.

% 3FHL
\bibitem[Ajello et al.(2017)]{Ajello-2017} Ajello, M. \& others\ 2017, \apj, 232, 18

% THOR
\bibitem[Anderson et al.(2017)]{Anderson-2017} Anderson, L. D. \& Wang, Y. \& Bihr, S. et al.\ 2017, A&A, 605, A58.

% HESS source
\bibitem[Angüner et al.(2017)]{Anguner-2017} Angüner, E. O. \& Casanova, S. \& Oya I. \& Aharonian, F. \& Bordas, P. \& Ziegler, A.\ 2017, Proceedings of 35th ICRC, 1708.04844

% XSPEC
\bibitem[Arnaud(1996)]{Arnaud-1996} Arnaud, K.~A.\ 1996, Astronomical Data Analysis Software and Systems V, 17.

% Cannonball
\bibitem[Albert et al.(2021)]{Albert-2021}Albert, A. et al.\ 2020, preprint.

% HENDRICS timing paper 
\bibitem[Bachetti et al.(2015)]{Bachetti-2015} Bachetti, M., Harrison, F. A., Cook, R., et al.\ 2015, ApJ, 800, 109

% Classic radiative processes
\bibitem[Blumenthal \& Gould(1970)]{Blumenthal-1970} Blumenthal, G.~R., \& Gould, R.~J.\ 1970, Reviews of Modern Physics, 42, 237.

% Leptonic UHC emission
\bibitem[Breuhaus et al.(2020)]{Breuhaus-2020} Breuhaus, M. \& Hahn, J. \& Romoli, C. \& Reville, B. \& Giacinti, G. \& Tuffs, R. \& Hinton, J. A.\ 2020, \apj, preprint.

% Chang HESS J1357
\bibitem[Chang et al.(2012)]{Chang-2012} Chang, C., Pavlov, G.~G., Kargaltsev, O., et al.\ 2012, \apj, 744, 81. doi:10.1088/0004-637X/744/2/81

% DA 495
\bibitem[Coerver et al.(2019)]{Coerver-2019} Coerver, A. \& Wilcox, P. \& Zhang, H. \& Dingus, B. L. \& Gotthelf, E. V. \& Hailey, C. J. \& Humensky, T. B. \& Kaaret, P. \& Li, H. \& Mori, K. \& et al.\ 2019, \apj, 878, 2.

% ISM magnetic field
\bibitem[Crutcher(2012)]{Crutcher-2012} Crutcher, Richard M.\ 2012, Annual Review of Astronomy and Astrophysics, 50, 29-63.

% Davidson Galactic center
\bibitem[Davidson et al.(1992)]{Davidson-1992} Davidson, J.~A., Werner, M.~W., Wu, X., et al.\ 1992, \apj, 387, 189.

% Duvidovich
\bibitem[Duvidovich et al.(2019)]{Duvidovich-2019} Duvidovich, L. \& Giacani, E. \& Castelletti, G. \& Petriella, A. \& Supán, L.\ 2019, A&A, 623, A115.

% Sherpa
\bibitem[Fruscione et al.(2006)]{sherpa} Fruscione, A. \& McDowell, J.~C. \& Allen, G.~E. et al.\ 2006, Proc. SPIE, 6270, 62701V.

% Yosi's model
\bibitem[Gelfand et al.(2009)]{Gelfand-2009} Gelfand, J.~D. \& Slane, P.~O. \& Zhang, W.\ 2009, \apj, 703, 2051. doi:10.1088/0004-637X/703/2/2051

% Gelfand 2009
%\bibitem[Gelfand et al.(2009)]{Gelfand-2009} Gelfand, Joseph D \& Slane, Patrick O \& Zhang, Weiqun\ 2009, \apj, 703, 2051.

% Gelfand Modelling PWNe
\bibitem[Gelfand(2017)]{Gelfand-2017} Gelfand, J. D.\ 2017, 161.

% Ginzburg 1965
%\bibitem[Ginzburg \& Syrovatskii(1965)]{Ginzburg-1965} Ginzburg, V. L. and Syrovatskii, S. I.\ 1965, \araa, 3, 297.

% Gotthelf
\bibitem[Gotthelf(2004)]{Gotthelf-2004} Gotthelf, E.~V.\ 2004, Young Neutron Stars and Their Environments, 218, 225.

% Fermi HESS 1826-134 detection
\bibitem[Grondin et al.(2011)]{Grondin-2011} Grondin, M.-H. \& Funk, S. \& Lemoine-Goumard, M., et al.\ 2011, \apj, 738, 42.

% Hydrodynamical balance and shock formation
\bibitem[Harding \& Gaisser(1990)]{Harding-1990} Harding, A.~K., \& Gaisser, T.~K.\ 1990, \apj, 358, 561.

% NuSTAR main ref
\bibitem[Harrison et al.(2013)]{Harrison-2013} Harrison, F.~A. \& Craig, W.~W. \& Christensen, F.~E., et al.\ 2013, \apj, 770, 103.

% HESS Collaboration 2018
\bibitem[Abdalla et al.(2018)]{Abdalla-2018} H.~E.~S.~S. Collaboration \& H.  Abdalla, \& A. Abramowski, \& F. Aharonian, \& F. Ait Benkhali, \& E. O.  Angüner, et al.\ 2018, A&A, 612, A1.

% Particle Transport J1825
\bibitem[Abdalla et al.(2019)]{Abdalla-2019} H.~E.~S.~S. Collaboration \& Abdalla, H. \& Aharonian, F. \& Ait Benkhali, F. \& Angüner, E. O. \& Arakawa, M. \& Arcaro, C. \& Armand, C. \& Arrieta, M. \& Backes, M. \& et al.\ 2019, A&A, 621, A116.

% HESS J1826-130 Extreme
\bibitem[Abdalla et al.(2020)]{Abdalla-2020} H.~E.~S.~S. Collaboration \& Abdalla, H. \& Adam, R., et al.\ 2020, \aap, 644, A112. doi:10.1051/0004-6361/202038851

%KN Regime IC
\bibitem[Hinton \& Aharonian(2007)]{Hinton-2007} Hinton, J. A. \& Aharonian, F. A.\ 2007, \apj, 657, 302-307.

% Sting-ray timing software
%\bibitem[Huppenkothen et al.(2016)]{Stingray-2016}
%Huppenkothen, D., {Bachetti}, M.,  {Stevens}, A.~L.,et al.\ 2016, Stingray: Spectral-timing software, Astrophysics
%Source Code Library, ascl:1608.001. 

% SNR secondary electrons and X-ray
\bibitem[Huang et al.(2020)]{Huang-2020} Huang, Yan \& Li, Zhuo \& Wang, Wei \& Zhao, Xiaohong\ 2020, Monthly Notices of the Royal Astronomical Society, 492, 4246–4253.

% Minuit
\bibitem[James \& Roos(1975)]{James-1975} James, F., \& Roos, M.\ 1975, Computer Physics Communications, 10, 343.

% Kang cooling timescale
\bibitem[Kang(2011)]{Kang-2011} Kang, Hyesung\ 2011, arXiv:1102.3109.

% Kargaltsev PWNe
\bibitem[Kargaltsev et al.(2017)]{Kargaltsev-2017} Kargaltsev, O. \& Pavlov, G. G. \& Klingler, N. \& Rangelov, B.\ 2017, Journal of Plasma Physics, 83, 5.

% Karpova
\bibitem[Karpova et al.(2019)]{Karpova-2019} Karpova, Anna V \& Zyuzin, Dmitry A \& Shibanov, Yuriy A\ 2019, Monthly Notices of the Royal Astronomical Society, 487, 1964–1972.

% Pulsar wind theory
\bibitem[Kirk et al.(2009)]{Kirk-2009} Kirk, J.~G. \& Lyubarsky, Y. \& Petri, J.\ 2009, Astrophysics and Space Science Library, 421.

% NuSTAR calibration
\bibitem[Madsen et al.(2015)]{Madsen-2015} Madsen, K.~K. \& Harrison, F.~A. \& Markwardt, C.~B., et al.\ 2015, The Astrophysical Journal Supplement Series, 220, 8.

% eventDisplay 
\bibitem[Maier \& Holder(2017)]{Maier-2017} Maier, G. \& Holder, J.\ 2017, International Cosmic Ray Conference, 301, 747.

% PWN magnetic field
\bibitem[Martin et al.(2014)]{Martin-2014} Martin, J. \& Torres, D. F. \& Cillis, A. \& de Oña Wilhelmi, E.\ 2014, Monthly Notices of the Royal Astronomical Society, 443, 138-145.

% KN effects
\bibitem[Moderski et al.(2005)]{Moderski-2005} Moderski, Rafal \& Sikora, Marek \& Coppi, Paolo S. \& Aharonian, Felix\ 2005, Monthly Notices of the Royal Astronomical Society, 363, 954-966.

% Mori dark accelerator
\bibitem[Mori et al.(2020)]{Mori-2020} Mori, Kaya \& An, Hongjun \& Feng, Qi \& Malone, Kelly \& Prado, Raul R. \& Schutt, Yve E. \& Dingus, Brenda L. \& Gotthelf, E. V. \& Hailey, Charles J. \& Hare, Jeremy et al.\ 2020, \apj, 897, 129.

% Vela R_TS
%\bibitem[Ng \& Romani(2004)]{Ng-2004} Ng, C.‐Y. \& Romani, Roger W.\ 2004, \apj, 601, 479–484.

% Cannonball
\bibitem[Nynka et al.(2013)]{Nynka-2013} Nynka, Melania \& Hailey, Charles J. \& Mori, Kaya \& Baganoff, Frederick K. \& Bauer, Franz E. \& Boggs, Steven E. \& Craig, William W. \& Christensen, Finn E. \& Gotthelf, Eric V. \& Harrison, Fiona A. et al.\ 2013, \apj, 778, 2041-8213.

% Review
\bibitem[Paredes \& Bordas(2019)]{Paredes-2019} Paredes, J.~M. \& Bordas, P.\ 2019, Rendiconti Lincei. Scienze Fisiche e Naturali, 1

% Fermi Hess
\bibitem[Principe et al.(2020)]{Principe-2020} Principe, G. \& Mitchell, A. M. W. \& Caroff, S.\2020, A&A, 640, A76

% G18.1-001 distance
\bibitem[Ranasinghe \& Leahy(2018)]{Ranasinghe-2018} Ranasinghe, S. \& Leahy, D.~A.\ 2018, \aj, 155, 204.

%Roberts
\bibitem[Roberts et al.(2007)]{Roberts-2007} Roberts, Mallory SE \& Gotthelf, EV \& Halpern, Jules P \& Brogan, Crystal L \& Ransom, Scott M\ 2007, arXiv preprint

% Romani pulsar torus
\bibitem[Romani et al.(2005)]{Romani-2005} Romani, R.~W. \& Ng, C.-Y. \& Dodson, R., et al.\ 2005, \apj, 631, 480.

% Rieger KN
\bibitem[Rieger et al.(2013)]{Rieger-2013} Rieger, F. M. \& de O˜na-Wilhelmi, E. \& Aharonian, F. A.\ 2013, Frontiers of Physics, 8, 714.

% Radiative processes in astrophysics
\bibitem[Rybicki \& Lightman(1979)]{Rybicki-1979} Rybicki, George B. \& Lightman, Alan P.\ 1979, John Wiley \& Sons.

% Slane PWNe 
\bibitem[Slane(2017)]{Slane-2017} Slane, Patrick\ 2017, Handbook of Supernovae, 2159–2179.

% Highest Energy HAWC Sources are Leptonic and Powered by Pulsars
\bibitem[Sudoh et al.(2021)]{Sudoh-2021} Sudoh, T. \& Linden, T. \& Hooper, D.\ 2021, arXiv:2101.11026

% Bohm diffusion D
\bibitem[Telezhinsky et al.(2012)]{Telezhinsky-2012} Telezhinsky, I. \& Dwarkadas, V. V. \& Pohl, M.\ 2012, A&A, 541, A153.

% Suzaku J1826-1334
\bibitem[Uchiyama et al.(2019)]{Uchiyama-2009} Uchiyama, Hideki \& Matsumoto, Hironori \& Tsuru, Takeshi Go \& Koyama, Katsuji \& Bamba, Aya\ 2009, Publications of the Astronomical Society of Japan, 61, S189–S196.

%Voisin gas
\bibitem[Voisin et al.(2016)]{Voisin-2016} Voisin, F., \& Rowell, G., \& Burton, M. G., \& Walsh, A. \& Fukui, Y. \& Aharonian, F.\ 2016, Monthly Notices of the Royal Astronomical Society, 458, 3.

% Naima 
\bibitem[Wilms et al.(2000)]{Wilms-2000} Wilms, J. \& Allen, A. \& McCray, R.\ 2000, \apj, 542, 914.

% Naima 
\bibitem[Zabalza(2015)]{Zabalza-2015} Zabalza, V.\ 2015, 34th International Cosmic Ray Conference (ICRC2015), 922.


\end{thebibliography}
